Lazard-style CAD and Equational Constraints

McCallum-style Cylindrical Algebra Decomposition (CAD) is a major improvement on the original Collins version, and has had many subsequent advances, notably for total or partial equational constraints. But it suffers from a problem with nullification. The recently-justified Lazard-style CAD does not have this problem. However, transporting the equational constraints work to Lazard-style does reintroduce nullification issues. This paper explains the problem, and the solutions to it, based on the second author's Ph.D. thesis and the Brown--McCallum improvement to Lazard. With a single equational constraint, we can gain the same improvements in Lazard-style as in McCallum-style CAD . Moreover, our approach does not fail where McCallum would due to nullification. Unsurprisingly, it does not achieve the same level of improvement as it does in the non-nullified cases. We also consider the case of multiple equational constraints.

==> macros.tex <==
%%% ZPT's macros
\newcommand{\bigO}{\mathcal{O}}
\newcommand{\true}{\text{\emph{true}}} % or \top
\newcommand{\false}{\text{\emph{false}}} % or \bot
\newcommand{\Kosta}{Ko\v{s}ta}
\newcommand{\VS}[3]{#1[#2\,/\hskip-2pt/\,#3]}
\newcommand{\algsubs}[3]{#1[#2\,/\,#3]}
\newcommand{\natNumbers}{\mathbb{N}}
\newcommand{\ints}{\mathbb{Z}}
\newcommand{\realNumbers}{\mathbb{R}}
\newcommand{\ratNumbers}{\mathbb{Q}}
\newcommand{\complexNumbers}{\mathds{C}}
\newcommand{\prefix}[2]{Q_{#2 - #1 + 1} x_{#2 - #1 + 1} \dots Q_{#2} x_{#2}}
\newcommand{\Qxi}[1]{Q_{#1} x_{#1}}
\newcommand{\Qxiblock}[2]{Q_{#1} x_{#1,1},\ldots,x_{#1,#2_{#1}}}
\newcommand{\prAnd}{\texttt{And}}
\newcommand{\prOr}{\texttt{Or}}
\newcommand{\rel}[3][\rho]{#2 \, #1 ~ #3}
\newcommand{\SCSQ}{\mathcal{SC}^2}
\newcommand{\Groebner}{Gr{\"o}bner}
\newcommand{\RootOf}{\mathop{\mathrm{RootOf}}\nolimits}
\newcommand{\myop}[1]{\mathop{\mathrm{#1}}\nolimits}
% algorithmicx formatting of variables, ``object membership'', function calls - modular
\newcommand{\var}[1]{\mathrm{#1}}
\newcommand{\objmem}{\mapsto}
\newcommand{\func}[1]{#1} % potentially \texttt, \textproc, or nothing
\newcommand{\objname}[1]{\texttt{#1}} % IQER, CADCell, etc.
\newcommand{\pckge}[1]{\texttt{#1}} % QuantifierElimination, RegularChains
\newcommand{\pluseq}{\mathrel{+}=}
\newcommand{\Cinc}{\texttt{++}}
\newcommand{\Cdec}{\texttt{--}}
\newcommand{\posints}{\mathds{N}_0}
\newcommand{\blankOutput}{\underline{\hspace{1em}}}
\newcommand{\realalgfun}[2]{\RootOf(#1,\var{index}=\var{real}[#2])}

